Lite Pose: Efficient Architecture Design for 2D Human Pose Estimation

Pose estimation plays a critical role in human-centered vision applications. However, it is difficult to deploy state-of-the-art HRNet-based pose estimation models on resource-constrained edge devices due to the high computational cost (more than 150 GMACs per frame). In this paper, we study efficient architecture design for real-time multi-person pose estimation on edge. We reveal that HRNet's high-resolution branches are redundant for models at the low-computation region via our gradual shrinking experiments. Removing them improves both efficiency and performance. Inspired by this finding, we design LitePose, an efficient single-branch architecture for pose estimation, and introduce two simple approaches to enhance the capacity of LitePose, including Fusion Deconv Head and Large Kernel Convs. Fusion Deconv Head removes the redundancy in high-resolution branches, allowing scale-aware feature fusion with low overhead. Large Kernel Convs significantly improve the model's capacity and receptive field while maintaining a low computational cost. With only 25% computation increment, 7x7 kernels achieve +14.0 mAP better than 3x3 kernels on the CrowdPose dataset. On mobile platforms, LitePose reduces the latency by up to 5.0x without sacrificing performance, compared with prior state-of-the-art efficient pose estimation models, pushing the frontier of real-time multi-person pose estimation on edge. Our code and pre-trained models are released at https://github.com/mit-han-lab/litepose.

==> cvpr/Figure/Figure-3-Advantage/Figure.tex <==
\begin{figure*}
\centering
	\includegraphics[width=\linewidth]{cvpr/Figure/Figure-3-Advantage/Figure-Adv.pdf}
\caption{\textbf{(a)} The performance improves as we gradually shrink the \textit{HigherHRNet} to \textit{Shrink3} and make it becomes increasingly single-branch-like. \textbf{(b)} Compared with the \textbf{multi-branch} HigherHRNet~\cite{cheng2020higherhrnet}, though our \textbf{single-branch} \textit{Lite Pose} takes more computational cost, it achieves similar latency on Qualcomm Snapdragon 855 with much higher performance.} 
\label{fig:3-advantage}
\end{figure*}


==> cvpr/Figure/Figure-5-Pretrain/Figure.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-33pt}
\begin{center}
	\includegraphics[height=0.33\textwidth]{cvpr/Figure/Figure-5-Pretrain/Figure-Pre.pdf}
\end{center}
\vspace{-10pt}
\caption{Pre-train ablations. With the help of pre-training trick, the model achieves higher performance and lower AE Loss.}
\label{fig:5-pretrain}
\vspace{-10pt}
\end{wrapfigure}


==> cvpr/Table/Table-AppLat.tex <==
% \begin{table}[h]
% \setlength{\tabcolsep}{8pt}
%   \centering
%   \begin{tabular}{lcccccccccc}
%     \toprule
%         \multirow{2}{*}{Model} & \multicolumn{2}{\multirow{2}{*}{\#MACs}} & \multicolumn{3}{\multirow{2}{*}{AP ($\uparrow$)}} & \multicolumn{6}{c}{Latency (ms)}  \\
%     \cmidrule(r){6-11} 
%     & & & & & \multicolumn{2}{c}{PyTorch}&TensorRT&AutoTVM\\
%     % \midrule
%     % HigherHRNet-W24 &24.1G&57.4 &443.2 &279.3& 344.4\\
%     % \textbf{LitePose (Ours)}&\textbf{5.0G}&\textbf{58.3}&\textbf{344.2}& 285.0 &\textbf{96.5}\\
%     \bottomrule
%   \end{tabular}
%   \vspace{5pt}
%   \caption{Comparisons between \textit{HigherHRNet} and \textit{LitePose}. The AP is measured on CrowdPose dataset. And the latency is measured on NVIDIA Jetson Nano GPU.}
%   \label{tab:applat}

% \end{table}

\begin{table}[h]
\setlength{\tabcolsep}{3.5pt}
  \centering
  \begin{tabular}{lccccc}
    \toprule
        \multirow{2}{*}[\multirowcenter]{Model} & \multirow{2}{*}[\multirowcenter]{\#MACs} & \multirow{2}{*}[\multirowcenter]{AP ($\uparrow$)} & \multicolumn{3}{c}{Latency (ms)}  \\
    \cmidrule(r){4-6} 
    & & & PyTorch&TensorRT&AutoTVM~\cite{chen2018tvm,zheng2020ansor}\\
    \midrule
    HigherHRNet-W24 &25.3G  & 57.4 & 443.2  & \textbf{279.3}  & 344.4 \\
    \textbf{LitePose (Ours)}&\textbf{5.0G} (\textbf{5.1}$\times$)& \textbf{58.3} (+\textbf{0.9}) &\textbf{344.2} (\textbf{1.3}$\times$)& 285.0 (1.0$\times$) &\textbf{96.5} (\textbf{3.6}$\times$)\\
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \caption{Latency comparisons between \textit{HigherHRNet} and \textit{LitePose} with different inference engines on Jetson Nano GPU. AP is measured on CrowdPose dataset~\cite{li2019crowdpose}. Lite Pose reduces the computation of HigherHRNet by 4.8$\times$, and achieves 3.6$\times$ speedup with AutoTVM~\cite{chen2018tvm,zheng2020ansor}. }
  \label{tab:applat}

\end{table}

==> cvpr/Table/Table-DEKR.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{4.5pt}
  \centering
  \begin{tabular}{llllll}
    \toprule
    Model&\#Params&\#MACs&AP\\
    \midrule
    LitePose-XS&1.7M&1.2G&49.5\\
    LitePose-S&2.7M&5.0G&58.3\\
    DEKR-12&4.3M&7.4G&56.3\\
    DEKR-8&2.0M&3.9G&51.0\\
    \bottomrule
  \end{tabular}
  \caption{Comparison results on CrowdPose. The number in model name means the number of base channel (\eg, \textit{16} in \textit{DEKR-16}). We cannot provide the latency results because the deformable convs used in DEKR are not supported by many inference engines.}
  \label{tab:dekr}
\end{table}

==> cvpr/Table/Table-Diff.tex <==
% \begin{table}[h]
% \small
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \begin{tabular}{lcccccc}
%     \toprule
%     Model&\multicolumn{2}{c}{\#Params}&\multicolumn{2}{c}{\#MACs}& \multicolumn{2}{c}{\#AP}\\
%     \midrule
%     Hourglass\cite{newell2016stacked} & 278M & -- &207G & -- & 56.6 & --\\
%     LitePose-S&2.7M & 103$\times$& 5.0G & 41$\times$& 56.7& $+0.1$\\
%     \bottomrule
%   \end{tabular}
%   \caption{\textit{LitePose-S} \vs U-Net-style \textit{Hourglass} on COCO \textit{test-dev}. \textit{LitePose} could achieve the same AP with $103\times$ less parameters and $41\times$ less \#MACs.}
%   \label{tab:diff}
% \end{table}

% \begin{table}[h]
% \small
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \begin{tabular}{lcccccc}
%     \toprule
%     Model&\multicolumn{2}{c}{\#Params}&\multicolumn{2}{c}{\#MACs}& \multicolumn{2}{c}{\#AP}\\
%     \midrule
%     Hourglass\cite{newell2016stacked} & 278M & -- &207G & -- & 56.6 & --\\
%     LitePose-S&2.7M & 103$\times$& 5.0G & 41$\times$& 56.7& $+0.1$\\
%     \bottomrule
%   \end{tabular}
%   \caption{\textit{LitePose-S} \vs U-Net-style \textit{Hourglass} on COCO \textit{test-dev}. \textit{LitePose} could achieve the same AP with $103\times$ less parameters and $41\times$ less \#MACs.}
%   \label{tab:diff}
% \end{table}

\renewcommand \arraystretch{1.}
\begin{table}[h]
\setlength{\tabcolsep}{2pt}
\small\centering
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}[\multirowcenter]{Model} &  \multicolumn{2}{c}{\#Params} & \multicolumn{2}{c}{\#MACs} & \multicolumn{2}{c}{AP ($\uparrow$)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& Value & Ratio & Value & Ratio & Value & Increase \\
\midrule
Hourglass & 278M & -- & 207G & -- & 56.6 & -- \\
\textbf{LitePose-S (Ours)} & \textbf{2.7M} & $103\times$ & \textbf{5.0G} & $41\times$ & \textbf{56.7} & $+0.1$ \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{\textit{LitePose-S} \vs U-Net-style \textit{Hourglass} on COCO \textit{test-dev}. \textit{LitePose} achieves better AP with much fewer \#Params and \#MACs.}
\vspace{-10pt}
\label{tab:diff}
\end{table}

==> cvpr/Table/Table-Dilated.tex <==
\begin{table}[h]
\small
\setlength{\tabcolsep}{4.5pt}
  \centering
  \begin{tabular}{lccccc}
    \toprule
    Setting & Dilation & \#Params & \#MACs&AP ($\uparrow$)\\
    \midrule
    % $3 \times 3$ Dilated Conv & 1.2M & 1.0G & 31.3 \\
    $3 \times 3$ Dilated Conv & 3 & 1.8M & 1.4G & 35.3 \\
    % \midrule
    $\mathbf{7 \times 7}$ \textbf{Conv (Ours)} & 1 & \textbf{1.7M} & \textbf{1.2G} & \textbf{49.5} \\\bottomrule
  \end{tabular}
%   \caption{Large kernel size is more effective than dilated conv in bottom-up pose estimation. \muyang{which dataset}}
    \vspace{-5pt}
    \caption{Our $7 \times 7$ conv could achieve a much higher AP on CrowdPose with less parameters and MACs.}
  \vspace{-15pt}
  \label{tab:dilated}
\end{table}

==> cvpr/Table/Table-Fusion.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{4.5pt}
  \centering
  \begin{tabular}{llllll}
    \toprule
    Model&Type of Head&\#Params&\#MACs&Pre-train&AP\\
    \midrule
    LitePose-Prune-S&Fusion Deconv&1.71M&4.69G&N&54.7\\
    LitePose-Prune-S&Simple Deconv&1.67M&4.06G&N&47.1\\
    \bottomrule
  \end{tabular}
  \caption{Fusion ablations. The results are measured on the CrowdPose dataset~\cite{li2019crowdpose}. Type ``Simple Deconv'' means the head does not utilize the low-level features generated by the backbone.}
  \label{tab:fusion}
\end{table}

==> cvpr/Table/Table-Larger-Kernel.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{4.5pt}
  \centering
  \begin{tabular}{llllll}
    \toprule
    Model&Kernel Size&\#Params&\#MACs&Pre-train&AP\\
    \midrule
    LitePose-Prune-S&$7\times 7$&1.71M&4.69G&N&54.7\\
    LitePose-Prune-S&$5\times 5$&1.48M&4.14G&N&50.7\\
    LitePose-Prune-S&$3\times 3$&1.33M&3.77G&N&41.7\\
    \bottomrule
  \end{tabular}
  \caption{Kernel size ablations. The results are measured on the CrowdPose dataset~\cite{li2019crowdpose}.}
  \label{tab:larger-kernel}
\end{table}

==> cvpr/Table/Table-Latency.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{4.5pt}
  \centering
  \begin{tabular}{lllll}
    \toprule
        \multirow{2}{\multirowcenter}{Model} & \multicolumn{2}{c}{Latency} &  \multirow{2}{\multirowcenter}{\#MACs} & \multirow{2}{\multirowcenter}{AP}  \\
    \cmidrule(r){2-3} 
    &Nano GPU&Intel CPU\\
    \midrule
    HigherHRNet-W16&990.2ms&\yihan{TODO}&12.50G&50.4\\
    LitePose-Prune-L&751.7ms&\yihan{TODO}&15.28G&62.1\\
    \bottomrule
  \end{tabular}
  \caption{Latency comparison results. In this table, we use three different metrics to evaluate the efficiency of different models. We also list the performance of each model on CrowdPose~\cite{li2019crowdpose}. The naming rule of models can be checked in Figure~\ref{fig:shrink} and Section \ref{sec:4.3}}
  \label{tab:latency}

\end{table}

==> cvpr/Table/Table-MACs.tex <==

\begin{table}[t]
\setlength{\tabcolsep}{4.5pt}
  \centering
  \begin{tabular}{cccc}
    \toprule
    Model&\#Params&\#MACs\\
    \midrule
    PersonLab&68.7M&405.5G\\
    Hourglass&277.8M&206.9G\\
    OpenPose&25.9M&160.0G\\
    HigherHRNet-W48&63.8M&155.1G\\
    \textbf{LitePose (Ours)} &\textbf{2.7M} & \textbf{5.0G}\\
    \bottomrule
  \end{tabular}
  \vspace{2mm}
  \label{tab:MACs}
   \vspace{-15pt}
\end{table}

==> cvpr/Table/Table-Pretrain.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{4.5pt}
  \centering
  \begin{tabular}{llllll}
    \toprule
    Model&\#Params&\#MACs&AE Loss~\cite{newell2016associative}&Pre-train&AP\\
    \midrule
    LitePose-Prune-S&1.71M&4.69G&7.891e-5&Y&56.1\\
    LitePose-Prune-S&1.71M&4.69G&8.329e-5&N&54.7\\
    \bottomrule
  \end{tabular}
  \caption{Pre-train ablations. In this table, we show the performance improvement by pretain. With more accurate heatmap prediction knowledge, the model can achieve higher performance (+1.4AP) with more accurate associate embedding~\cite{newell2016associative} (-0.438 AE loss).}
  \label{tab:pretrain}
\end{table}

==> cvpr/Table/Table-Shrinking.tex <==
\begin{table}[h]
\renewcommand*{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}
\small\centering
  \begin{tabular}{lllllll}
    \toprule
    \multirow{2}{\multirowcenter}{Model} & \multicolumn{4}{c}{\#Blocks in Stages} & \multirow{2}{\multirowcenter}{\#MACs} & \multirow{2}{\multirowcenter}{AP}  \\
    \cmidrule(r){2-5} 
    &Stem&Stage2&Stage3&Stage4\\
    \midrule
    HigherHRNet-W16-512&4&[4,4]&[4,4,4]&[4,4,4,4]&12.50G&50.4\\
    HigherHRNet-W16-512-Shrink1&4&[3,4]&[2,3,4]&[1,2,3,4]&10.12G&51.0\\
    HigherHRNet-W18-512-Shrink2&4&[1,4]&[1,1,4]&[1,1,1,4]&10.02G&51.8\\
    HigherHRNet-W18-512-Shrink3&4&[0,4]&[0,0,4]&[0,0,0,4]&9.15G&53.0\\
    \bottomrule
  \end{tabular}
%     \begin{tabular}{llllllll}
%     \toprule
%     \multirow{2}{\multirowcenter}{\#Base Channel} & \multicolumn{4}{c}{\#Blocks in Stages} & \multirow{2}{\multirowcenter}{\#Params} & \multirow{2}{\multirowcenter}{\#MACs} & \multirow{2}{\multirowcenter}{AP}  \\
%     \cmidrule(r){2-5} 
%     &Stem&Stage2&Stage3&Stage4\\
%     \midrule
%     16&4&[4,4]&[4,4,4]&[4,4,4,4]&7.21M&12.50G&50.4\\
%     16&4&[3,4]&[2,3,4]&[1,2,3,4]&6.71M&10.12G&51.0\\
%     \midrule
%     16&4&[1,4]&[1,1,4]&[1,1,1,4]&6.04M&8.36G&49.8\\
%     18&4&[1,4]&[1,1,4]&[1,1,1,4]&7.62M&10.02G&51.8\\
%     \midrule
%     18&4&[0,4]&[0,0,4]&[0,0,0,4]&7.38M&9.15G&53.0\\
%     20&4&[0,4]&[0,0,4]&[0,0,0,4]&9.09M&10.78G&54.1\\
%     \bottomrule
%   \end{tabular}
  \caption{Shrinking Ablations of HigherHRNet~\cite{cheng2020higherhrnet} on CrowdPose dataset~\cite{li2019crowdpose}. In this table, we show the shrinking experiments in details. The number after "W" represent the number of base channel and the second number means the input resolution. For example, W16-512 means the number of base channel is 16 in the corresponding architecture, and the input resolution for such architecture is $512\times 512$. \muyang{Some conclusions of this table.}}
  \label{tab:shrinking}
\end{table}

==> cvpr/macros.tex <==
% \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}} 
\newcommand{\xpar}[1]{\noindent\textbf{#1}\ \ }
\newcommand{\vpar}[1]{\vspace{3mm}\noindent\textbf{#1}\ \ }

\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\sects}[1]{Sections~\ref{#1}}
\newcommand{\eqn}[1]{Equation~\ref{#1}}
\newcommand{\eqns}[1]{Equations~\ref{#1}}
\newcommand{\fig}[1]{Figure~\ref{#1}}
\newcommand{\figs}[1]{Figures~\ref{#1}}
\newcommand{\tab}[1]{Table~\ref{#1}}
\newcommand{\tabs}[1]{Tables~\ref{#1}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\fid}{Fr\'echet Inception Distance\xspace}
\newcommand{\lblfig}[1]{\label{fig:#1}}
\newcommand{\lblsec}[1]{\label{sec:#1}}
\newcommand{\lbleq}[1]{\label{eq:#1}}
\newcommand{\lbltbl}[1]{\label{tbl:#1}}
\newcommand{\lblalg}[1]{\label{alg:#1}}
\newcommand{\lblline}[1]{\label{line:#1}}

\newcommand{\ignorethis}[1]{}
\newcommand{\norm}[1]{\lVert#1\rVert_1}
\newcommand{\fcseven}{$\mbox{fc}_7$}

\renewcommand*{\thefootnote}{\fnsymbol{footnote}}

% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

\def\naive{na\"{\i}ve\xspace}
\def\Naive{Na\"{\i}ve\xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\iid{\emph{i.i.d}\onedot}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\def\vs{\textbf{\emph{vs}\onedot}}
\makeatother

\definecolor{citecolor}{RGB}{34,139,34}
\definecolor{mydarkblue}{rgb}{0,0.08,1}
\definecolor{mydarkgreen}{rgb}{0.02,0.6,0.02}
\definecolor{mydarkred}{rgb}{0.8,0.02,0.02}
\definecolor{mydarkorange}{rgb}{0.40,0.2,0.02}
\definecolor{mypurple}{RGB}{111,0,255}
\definecolor{myred}{rgb}{1.0,0.0,0.0}
\definecolor{mygold}{rgb}{0.75,0.6,0.12}
\definecolor{mydarkgray}{rgb}{0.66, 0.66, 0.66}


\newcommand{\supplement}[1]{\color{blue}{#1}}
\newcommand{\muyang}[1]{{\color{orange}{[}Muyang: #1{]}}}
\newcommand{\han}[1]{{\color{mydarkblue}{[}Han: #1{]}}}
\newcommand{\yihan}[1]{{\color{purple}{[}Yihan: #1{]}}}
\newcommand{\SH}[1]{{\color{red}{[}SH: #1{]}}}
\newcommand{\myparagraph}[1]{\paragraph{#1}}

\def\multirowcenter{-0.5\dimexpr \aboverulesep + \belowrulesep + \cmidrulewidth}
\renewcommand{\thefootnote}{\number\value{footnote}}

\newcommand\blfootnotetext[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnotetext{#1}%
  %\addtocounter{footnote}{-1}%
  \endgroup
}
